On Shapley Value in Data Assemblage Under Independent Utility

In many applications, an organization may want to acquire data from many data owners. Data marketplaces allow data owners to produce data assemblage needed by data buyers through coalition. To encourage coalitions to produce data, it is critical to allocate revenue to data owners in a fair manner according to their contributions. Although in literature Shapley fairness and alternatives have been well explored to facilitate revenue allocation in data assemblage, computing exact Shapley value for many data owners and large assembled data sets through coalition remains challenging due to the combinatoric nature of Shapley value. In this paper, we explore the decomposability of utility in data assemblage by formulating the independent utility assumption. We argue that independent utility enjoys many applications. Moreover, we identify interesting properties of independent utility and develop fast computation techniques for exact Shapley value under independent utility. Our experimental results on a series of benchmark data sets show that our new approach not only guarantees the exactness of Shapley value, but also achieves faster computation by orders of magnitudes.

==> latexmkrc <==
# vim: set filetype=perl:

$pdf_mode = 1;
set_tex_cmds('-synctex=1 -file-line-error %O %S');
$max_repeat = 5;

# File extensions to remove when cleaning
# Ref: https://www.gitignore.io/api/latex
my @clean_ext = qw(
  %R-blx.aux
  %R-blx.bib
  acn
  acr
  alg
  aux
  bbl
  bcf
  blg
  brf
  cb
  cb2
  cpt
  cut
  dvi
  fdb_latexmk
  fls
  fmt
  fot
  glg
  glo
  gls
  glsdefs
  idx
  ilg
  ind
  ist
  lb
  listing
  loa
  loe
  lof
  log
  lol
  lot
  lox
  nav
  out
  pdfsync
  pre
  run.xml
  snm
  soc
  synctex
  synctex(busy)
  synctex.gz
  synctex.gz(busy)
  tdo
  thm
  toc
  upa
  upb
  vrb
  xcp
  xdv
  xmpi
  xyc
  *-converted-to.*
  */*-converted-to.*
  */*/*-converted-to.*
  */*/*/*-converted-to.*
  */*/*/*/*-converted-to.*
  */*/*/*/*/*-converted-to.*
  */*/*/*/*/*/*-converted-to.*
  */*/*/*/*/*/*/*-converted-to.*
  */*/*/*/*/*/*/*/*-converted-to.*
  */*/*/*/*/*/*/*/*/*-converted-to.*
);
$clean_ext = join ' ', @clean_ext;

no warnings 'redefine';

# Overwrite `cleanup1` functions to support more general pattern in $clean_ext.
# Ref: https://github.com/e-dschungel/latexmk-config/blob/master/latexmkrc
sub cleanup1 {
    my $dir = fix_pattern( shift );
    my $root_fixed = fix_pattern( $root_filename );
    foreach (@_) {
        (my $name = (/%R/ || /[\*\?]/) ? $_ : "%R.$_") =~ s/%R/$dir$root_fixed/;
        unlink_or_move( glob( "$name" ) );
    }
}
